Multi-modal Agent Tuning: Building a VLM-Driven Agent for Efficient Tool Usage

The advancement of large language models (LLMs) prompts the development of multi-modal agents, which are used as a controller to call external tools, providing a feasible way to solve practical tasks. In this paper, we propose a multi-modal agent tuning method that automatically generates multi-modal tool-usage data and tunes a vision-language model (VLM) as the controller for powerful tool-usage reasoning. To preserve the data quality, we prompt the GPT-4o mini model to generate queries, files, and trajectories, followed by query-file and trajectory verifiers. Based on the data synthesis pipeline, we collect the MM-Traj dataset that contains 20K tasks with trajectories of tool usage. Then, we develop the T3-Agent via \underline{T}rajectory \underline{T}uning on VLMs for \underline{T}ool usage using MM-Traj. Evaluations on the GTA and GAIA benchmarks show that the T3-Agent consistently achieves improvements on two popular VLMs: MiniCPM-V-8.5B and {Qwen2-VL-7B}, which outperforms untrained VLMs by $20\%$, showing the effectiveness of the proposed data synthesis pipeline, leading to high-quality data for tool-usage capabilities.

==> figure/manuscript_preprint.tex <==

\section{Introduction}
\vskip -0.2in
Integrating external tools to solve diverse multi-modal tasks is a promising research direction towards multi-modal agents~\citep{suris2023vipergpt,gupta2023visual,gao2024clova,yuan2023craft,zhong2023viotgpt}.
Existing agents usually use a large language model (LLM) as the controller that generates plans via prompt engineering to call tools, achieving impressive performance in multiple domains, such as image editing~\citep{wu2023visual}, robotic manipulation~\citep{pmlr-v205-ichter23a}, question answering~\citep{shen2024hugginggpt}, video understanding~\citep{fan2024videoagent}, and desktop APPs~\citep{trivedi2024appworld}. 
Despite their success, prompt engineering faces limited reasoning abilities for tool usage in tackling practical tasks, as shown in~\cref{fig:teaser_example}. 
(1) The in-context examples in prompts only involve textual information, degrading the efficiency of tool usage in the multi-modal world.
For the query `How many dollars will I need to spend to buy a PS5 for each child?', the agent may select improper tools if it does not know what the two images depict.
(2) The pre-defined in-context examples are fixed and cannot tackle all tasks in the real world. 
For the task that requires searching for information from the web, the agent cannot use the proper tools, if in-context examples tend to use the `image\_qa' tool.
This motivates us to enhance the controller's reasoning ability for efficient tool usage.
% in diverse and complex tasks.


In this paper, we propose a multi-modal agent tuning method that automatically generates a large number of multi-modal tasks with tool-usage trajectories and tunes a vision-language model (VLM)~\citep{liu2024visual,chen2024internvl,yao2024minicpm} as the controller for powerful tool-usage reasoning.
Compared with LLM-driven agents, VLM-driven agents can utilize multi-modal information (such as required knowledge domains in the multi-modal data) instead of only using the query for reasoning, benefiting efficient tool usage~\citep{liu2024visualagentbench,wang2024mllm,sun2024details}. 
Many efforts are made to enhance specific capabilities of VLMs via finetuning, such as the chain-of-thought ability~\citep{hu2024visual}, grounding ability~\citep{peng2023kosmos}, and feedback-refining ability~\citep{li2024fire}.
This inspires us to construct a large number of multi-modal tool-usage data for VLM-driven agents, which improves the reasoning ability when using tools for real-world tasks.


In doing so, we need to overcome two challenges.
(1) Collecting multi-modal tasks is challenging. Tasks in the real world usually involve multiple tools for multiple files (images, textual files, videos, audio, and \emph{etc}). There are few off-the-shelf datasets for such tasks, and prompting models to generate natural and diverse queries with matched files is non-trivial.
(2) Generating trajectories is challenging. 
Due to the complexity of trajectories, existing methods usually manually define templates and fill in key information for trajectory generation. This will limit the diversity of synthesis data and cause weak generalization for real-world tasks. 



To overcome the above challenges, we introduce a novel tool-usage data synthesis pipeline that automatically generates a large number of multi-modal tool-usage data via three steps: query generation, file generation, and trajectory generation.
Concretely, we first prompt GPT-4o mini~\citep{2024GPT4OisionSC} to generate queries and analyze what files are needed to solve the queries.
Then, we produce files via two strategies.
If needed files are images, we search for them from existing image datasets; otherwise, we prompt GPT-4o mini to produce codes to generate the needed files.
Finally, we prompt a zero-shot agent to solve the generated tasks (\emph{i.e.}, queries and files) and collect trajectories, including the thoughts and codes in task solving.
To preserve the data quality, the generated tasks and trajectories are passed through two verifiers to discard low-quality data.
After that, we use these data to tune a VLM for efficient tool usage, through which one agent driven by the trained VLM could generate precise thoughts and codes for real-world tasks.


With the data generation pipeline, we construct MM-Traj, a dataset that contains 20K multi-modal tasks with tool-usage trajectories.
Based on MM-Traj, we introduce the T3-Agent, a VLM-driven agent in the ReAct framework~\citep{yao2023react}. The VLM controller of the T3-Agent 
% model~\citep{yao2024minicpm}, a popular VLM, as the controller, which 
is developed via \underline{T}rajectory \underline{T}uning for \underline{T}ool usage using MM-Traj.
We conduct comprehensive evaluations of the T3-Agent on the GTA~\citep{wang2024gta} and GAIA benchmarks~\citep{mialon2023gaia}, where two popular VLMs are used as the controller, that is MiniCPM-V-8.5B~\citep{yao2024minicpm} and {\color{red}Qwen-VL-7B}~\citep{wang2024qwen2}.
The T3-Agent consistently achieves improvements on the two VLMs and outperforms the untrained VLMs by $20 \%$. 
This indicates that our multi-modal agent tuning method enables agents a powerful tool-usage capability for practical tasks with complex and diverse trajectories.



% Compared with LLM-driven multi-modal agents, VLM-driven agents can utilize multi-modal information (such as the image type and involved knowledge domain as shown in Figure) in planning instead of only text, showing efficient tool usage in multiple domains, such as visual design~\citep{} and robotic manipulation~\citep{}. 
% However, current VLMs may fail to plan for real-world tasks that require complex tool-usage trajectories, possibly due to the lack of multi-modal chain-of-thought data, limiting the performance of agents. This prompts us to enhance VLMs for powerful multi-modal agents.


% To solve this issue, some efforts are made to generate tool-usage trajectories and enhance VLMs of agents by using the generated data for fine-tuning. 
% Despite their growing potential, their agents are usually hampered by the data volume and diversity, limiting their application in real-world tasks.
% They usually focus on cases with one or few tools in the trajectories and involve human involvement for predefined trajectory templates, causing insufficient training data and weak generalization for VLMs that use these training data.
% For example, as shown in~\citep{}, the VLM-driven agents trained on collected 1K data still have a large margin with agents using close-source LLM (such as GPT-4).
% This inspires us to construct multi-modal trajectories for VLM-driven agents.




% To this end, we propose 
% % a tool-usage trajectory synthesis pipeline,
% a multi-modal agent tuning method as shown in Figure, 
% which automatically generates a large number of multi-modal tool-usage trajectories and enhances VLMs of agents by using the generated data for fine-tuning. 
% Synthesizing tool-usage data has shown effectiveness in LLM-driven agents, which generate a trajectory for real-world tasks via in-context learning~\citep{}, manual design~\citep{}, or data conversation~\citep{}, data verification. 
% The high-quality synthetic data can significantly improve the tool-usage capability for agents, making general tool-usage for complex real-world tasks, showing a feasible way for VLM-driven agents.
% inspiring us to construct multi-modal trajectories for VLM-driven agents.




% Pipeline. 

% Tune agent


In summary, our contributions are three-fold. (1) We propose a multi-modal agent tuning method that automatically generates a large number of multi-modal tasks with trajectories and tunes VLMs using the generated data for powerful tool usage. (2) We introduce MM-Traj, a multi-modal tool-usage dataset that contains 20K tasks across diverse knowledge domains with 15K files and high-quality trajectories. (3) We develop the T3-Agent, a multi-modal tool-usage agent that significantly improves the tool usage performance on two popular benchmarks: GTA and GAIA.




\section{Related Work}
\vskip -0.1in
\subsection{Multi-Modal Agent}
\vskip -0.1in
Using external tools to address complex tasks is an important ability for multi-modal agents. According to different controllers, existing agents can be categorized into LLM-driven agents and VLM-driven agents.
LLM-driven agents utilize powerful LLMs as the controller and produce pseudo code~\citep{gupta2023visual,gao2024clova}, python code~\citep{suris2023vipergpt,yuan2023craft}, or JSON format~\citep{shen2024hugginggpt} to call tools via one-step reasoning. Considering the complexity of practical tasks, some methods~\citep{yang2023mm,fan2024videoagent,yang2024doraemongpt} empower the agent with step-by-step reasoning, which allocates tools based on observations of previous steps.
Compared with LLM-driven agents, VLM-driven agents are more efficient in task solving, since the VLM controller can utilize information from visual data in tool usage, showing superior performance in visual design~\citep{sasazawa2024layout}, web search~\citep{zheng2024gpt}, image editing~\citep{wang2024genartist}, embodied scenario~\citep{zheng2023steve}, robotic manipulation~\citep{sun2024details}, and \emph{etc}.
However, VLM-driven agents have a weaker reasoning ability, compared with LLM-driven agents.
Thus, several works synthesize training data to tune open-source VLMs for general tool usage~\citep{wang2024mllm,liu2023llava,liu2024visualagentbench}.
Due to the challenges of trajectory generation, existing methods mainly focus on simple tasks requiring one or two tools, and only synthesize a small amount of data (\emph{e.g.}, 1K in~\citep{liu2024visualagentbench}).
Different from them, our T3-Agent is tuned using scaled-up multi-modal data with complex tool-usage trajectories, through which our agent could solve more practical tasks with strong tool-usage capability.


% Some methods focus on tasks that only require few tools~\citep{wang2024mllm,liu2023llava}, and a recent work~\citep{} tries to build a VLM-driven agent via generating about 1K data.
% Even though, multi-modal agents still cannot achieve satisfied performance on complex tasks with complex tool-usage trajectories.



\subsection{Tool-Usage Dataset}
\vskip -0.1in
Several tool-usage datasets have been established for agents, such as APIBank~\citep{li2023api}, Toolalpaca~\citep{tang2023toolalpaca}, ToolBench~\citep{qin2023toolllm}, AnyTool~\citep{du2024anytool}, 
agentohana~\citep{zhang2024agentohana}, APIGen~\citep{liu2024apigen}, and AgentInstruct~\citep{zeng2023agenttuning}.
The above datasets contain little multi-modal data (\emph{e.g.}, images, videos, and audios) that are commonly encountered in the real world. 
Thus, to evaluate the performance of agents in solving multi-modal tasks, some multi-modal agent benchmarks have been built, such as the GUI benchmarks: OSWorld~\citep{xie2024osworld} and MMInA~\citep{zhang2024mmina}, multi-modal question answering benchmarks: GAIA~\citep{mialon2023gaia}, GTA~\citep{wang2024gta}, and m\&m'~\citep{ma2024m}, and comprehensive benchmarks: AgentBench~\citep{liu2023agentbench} and AgentGym~\citep{xi2024agentgym}.
In addition, some efforts are paid to synthesize trajectory data using LLMs to improve the tool-usage ability of multi-modal agents. 
DEDER~\citep{choiembodied} resorts to in-context learning to generate trajectories, through which the chain-of-thought reasoning ability is distilled from LLMs to a small model.
Lumos~\citep{yin2024agent} converts ground-truth reasoning steps in existing
benchmarks into the expected format of tool-usage trajectories.
TASKBENCH~\citep{shen2023taskbench} samples trajectories from a predefined graph, and then generate queries.
MLLM-Tool~\citep{wang2024mllm} and LLaVA-plus~\citep{liu2023llava} collect trajectories based on image and tool descriptions. VisualAgentBench~\citep{liu2023agentbench} manually designs trajectory templates to collect data.
Different from the above methods that usually focus on simple and predefined trajectories, or rely on queries in off-the-shelf datasets,
% (MLLM-Tool and LLaVA-plus only use one or two tools in a task, and VisualAgentBench predefines templates for the trajectories), 
our data collection pipeline does not have any constraints, which generates diverse tasks and complex trajectories, improving the volume, complexities, naturalness, and diversity of the tool-usage dataset.


\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.9\linewidth]{figure/data_generation.pdf}
    \vskip -0.15in
    \caption{The pipeline for data generation.}
    \vskip -0.3in
    \label{fig:data_gathering}
\end{center}
\end{figure}


\section{Data Collection}
\vskip -0.1in
\subsection{Formulation}
\vskip -0.1in

\textbf{Data Synthesis Pipeline.} The proposed data synthesis pipeline is shown in~\cref{fig:data_gathering}, including three steps: query generation, file generation, and trajectory generation. To preserve the quality of data, we design a query-file verifier and a trajectory verifier to discard low-quality data. 


\textbf{Data format.}
We format the multi-modal tool-usage data as $\{ F_{\text{opt}}, Q, T, C, O, A \}$, where $F_{\text{opt}}$ denotes the multi-modal files, $Q$ means the query, $T$ mean the generated thought (\emph{i.e.}, plans to call tools), and $C$ means the generated code, $O$ means observation (outputs of using tools), and $A$ means the ground truth answer. $_{\text{opt}}$ means that the files are optional, \emph{i.e.}, some queries do not involve files. 


The query $Q$ could be divided into two categories, question answering and image generation, where the answer $A$ would be some descriptive texts for the former and images for the latter.
In our setting, $F$ includes 11 types of files, such as JPG, PDF and PPTX files (details in Appendix). Considering that solving one real-world task may require multiple steps involving multiple tools, $T$, $C$, and $O$ can be represented by the integration of thought, code, and observation in multiple steps, and the data format is reformulated as $\{ F_{\text{opt}}, Q, \{t_1, \cdots, t_n\}, \{c_1, \cdots, c_n\}, \{o_1, \cdots, o_n\}, A \}$, where $t_i$, $c_i$, and $o_i$ indicate the thought, code, and observation in the $i$-step respectively, and there are $n$ steps in total. 
The thought, code, and observation are composed of a trajectory $\{t_1, c_1, o_1, \cdots, t_n, c_n, o_n\}$ of $n$ steps to solve the query.





\textbf{Image source.} 
Visual information plays an important role in multi-modal tasks.
To enhance the diversity and comprehensiveness of our tool-usage data, we compile about 93K image-captioning pairs from 8 source datasets, including ChartQA~\citep{masry2022chartqa}, COCO~\citep{lin2014microsoft}, LLaVA~\citep{wang2023see}, SAM~\citep{kirillov2023segment}, TextVQA~\citep{singh2019towards}, Web-Celebrity~\citep{liu2015faceattributes}, Web-Landmark~\citep{weyand2020GLDv2}, and WikiArt~\citep{saleh2015large}.
These datasets cover multiple multi-modal tasks: visual question answering, chart/table/document analysis, science question answering, and \emph{etc}.
We use the ShareGPT4V model~\citep{chen2023sharegpt4v} to produce captions for each collected image.


\subsection{Query Generation}
\vskip -0.1in
Our goal is to generate a large number of diverse, practical, and feasible queries.
We manually write some seed queries by brainstorming and double-checking them to ensure their practicality.
In each step of query generation, 
we feed several randomly sampled seed queries, tools with descriptions, and a designed prompt to the GPT-4o mini model that generates multiple queries. 
Adding tool descriptions to the prompt makes GPT-4o mini better understand the desirable queries, improving the feasibility of generated queries.
We tune the hyperparameters (such as temperature) of GPT-4o mini to improve the diversity of generation.
 % 
% We ask the GPT-4o mini model to generate 23K queries at once, calling a total of *** times, resulting in a total of *** queries being generated.





\subsection{Multi-modal File Generation}
\vskip -0.1in
Different from existing multi-modal data synthesis methods that first sample multi-modal files (images in most cases) from off-the-shelf datasets and then feed the files to language models (\emph{e.g.}, ChatGPT) for query generation, we opt to first generate queries without files and then produce relevant files for the queries. 
The reasons are two aspects. 
(1) Practical tasks usually involve not only images but also other multi-modal files, such as DOCX, PPTX, XLSX, and PDF files. It is challenging to construct off-the-shelf datasets that contain enough files for real-world tasks.
(2) Tasks are usually based on multiple files instead of only one, while randomly sampled files may have weak relevance and feeding them to language models usually produces non-natural queries. It is non-trivial to design a standard to automatically sample relevant files for query generation.
(3) Using existing files to generate queries may limit the knowledge domain, decreasing the diversity of tasks. In contrast, generating files based on generated queries may lead to more diversity.


Concretely, for each generated query, we prompt GPT-4o mini to output the needed file type and file content. The files are divided into two categories: images and others. 
For needed images, we use the BGE model~\citep{bge-m3} to extract textual embeddings of the file content and compare its similarities with collected source images from off-the-shhackelf datasets. The top similar images are collected for the query.
For other needed files, we prompt GPT-4o mini to extend the file content and generate Python code to produce the files.



\subsection{Zero-Shot Agent Inference}
\vskip -0.1in
Trajectories are collected by prompting a zero-shot agent (without training) to solve our generated tasks (\emph{i.e.}, queries and files). 
We utilize the framework of ReAct agents~\citep{yao2023react}, where GPT-4o mini is employed as the controller. It solves the query into multiple steps and generates thought and code for each step based on the observations of previous steps.
We collect trajectories whose code can be executed, including the thoughts, codes, and observations of all steps.
The details of the agent can be found in Section~\cref{section:tools} and~\cref{section:prompt}.

\subsection{Data Verification}
\vskip -0.1in

To preserve the quality of generated tool-usage data, we design a query-file verifier and a trajectory verifier to discard low-quality data. {\color{red}Using LLMs to verify the quality of LLM outputs has shown effectiveness in multiple methods, such as verifying the generated instructions~\citep{wang2023self} and verifying the generated plans~\citep{liu2024apigen}. Inspired by them, we argue that using LLMs can also verify the synthetic tasks and trajectories.}

\textbf{Query-file verifier.} Considering that the generated queries may be infeasible to solve and the produced files may not match the queries, the query-file verifier filters out low-quality query-file pairs. 
We prompt GPT-4o mini as the verifier based on the following factors: (1) whether the query and files are relevant; (2) whether the files contain enough information to solve the query; and (3) whether the query can be solved based on the given tools.

\textbf{Trajectory verifier.}
Similarly, we prompt GPT-4o mini as the trajectory verifier based on the following factors: (1) the trajectory should use the provided tools as much as possible; (2) the trajectory should be reasonable, that is, the trajectory should align with the object and context of the query; (3) the tool usage in the trajectory should consistent with the query and files; (4) the input arguments for tools in the trajectory should be correct; (5) the answer should be correctly summarized from observations of tool-usage; and (6) the final answer should be relevant to the query.


\subsection{MM-Traj Dataset}
\vskip -0.1in
Data that passes through the two verifiers is considered high-quality and collected in an MM-Traj dataset. In summary, we collect 23.5K data points from query generation and file generation. After passing through the two verifiers, 20K data points are left with 15K files.

{\color{red}\textbf{Scalability.} Note that our method can extend to additional modalities by incorporating more tools and leveraging advanced multi-modal models. For example, to extend our method to the video modality (MP4, MOV), we can integrate a video search model into the data synthesis pipeline (like the image modality), and apply a video-language model to the agent controller with powerful video processing models as tools. This approach ensures seamless adaptation to new modalities while maintaining efficiency and coherence.}


\begin{figure}[htbp]
\centering
    \subfigure[File type]{
  \includegraphics[width=0.48\textwidth]{figure/file_statistics}\label{fig:file_type}}
    \subfigure[Domain Knowledge]{
  \includegraphics[width=0.48\textwidth]{figure/topic_statistics_2}\label{fig:domain_knowledge}}
    \subfigure[Tool Statistic]{
  \includegraphics[width=0.48\textwidth]{figure/tool_statistics }\label{fig:tool_statistic}}
    \subfigure[{\color{red}Step Number}]{
  \includegraphics[width=0.48\textwidth]{figure/step_distribution.png}\label{fig:step_number}}
  \vskip -0.15in
  \caption{Data statistics on the MM-Traj dataset.}
  \label{fig:data_statistics1}
  \vskip -0.15in
\end{figure}


\subsubsection{Dataset Analysis}
% \vskip -0.1in
We provide four key statistics: file type, knowledge domain, step number, and used tools in the collected MM-Traj Dataset.
\textbf{File type.} We show the distribution of involved files in~\cref{fig:file_type}, which reflects the diversity of our dataset. MM-Traj covers more than 9 files, all of which are commonly encountered in the real world. Thus the T3-Agent trained on MM-Traj can handle practical tasks since the multi-modal knowledge is not limited to images in our lives.
\textbf{Knowledge domain.} We show the involved knowledge of the generated tasks in~\cref{fig:domain_knowledge}, which can be divided into 16 non-overlap categories, spanning across finance, environment, culture, health, history, food, and \emph{etc.}
Training in such data provides rich knowledge to use tools to solve diverse practical tasks.  
\textbf{Tools.} In~\cref{fig:tool_statistic}, We show the distributions of used tools in generated trajectories. The web search tool is the most commonly used tool, which is consistent with practical tasks requiring specific knowledge. Moreover, other tools are also widely used in our dataset.
\textbf{Step number.} We show the distributions of step numbers of generated trajectories in~\cref{fig:step_number}.
% Only a few tasks are solved in only two steps, showing the complexity of our dataset. 
Trajectories in the MM-Traj dataset have diverse step numbers. Most tasks require 2-6 steps to solve and some tasks require 7-8 steps, showing the complexity and diversity of our dataset. 






\section{T3-Agent}
\vskip -0.1in
\subsection{Workflow}
\vskip -0.1in
To handle practical tasks that require complex trajectories, we opt for the framework of the ReAct agent that performs step-by-step reasoning for tool usage based on observations of previous steps.
In each step, the agent generates thought and corresponding code to execute tools. 
Compared with other formats (\emph{e.g.}, JSON format), code is more flexible to handle different inputs and output types for various tools. Concretely, given a query $Q$ and files $F$, the $i$-step of the agent is formulated as
\begin{equation}
\begin{aligned}
t_i^{\star}, c_i^{\star} = \arg \max P(t_i, c_i| F_{\text{opt}}, Q, h_i), 
\end{aligned}
\end{equation}
where $t_i^{\star}$ and $c_i^{\star}$ are generated thought and code for the $i$-th step, and $h_i = \{ t_1,c_1,o_1,\cdots, t_{i-1},c_{i-1},o_{i-1} \}$ denotes the history (thought, code, and observation of previous steps).

\subsection{Tools}
\vskip -0.1in
We deploy real-executable tools for the agent instead of only providing tool names. Our tools are across multiple categories: web search, visual perception, image generation/editing, file understanding,  multi-modal understanding, and multiple Python packages, as shown in~\cref{table:tool_description}.

\begin{table}[t]
\caption{Used tools in the T3-Agent}
\vskip -0.15in
\label{table:tool_description}
\begin{center}
\begin{tabular}{c | c}
\hline 
\multicolumn{1}{c|}{\bf Tool name}  & \multicolumn{1}{c}{\bf Tool description} 
\\ \hline
Web search & Perform complicated web browsing to answer a question \\
Image question answering & Answer questions for queries based on attached images\\
File inspector & Answer questions for queries based on given files\\
Visual segmentation & Do instance segmentation on the given image\\
Object localization & Localize objects in given images and output the bounding boxes\\
Image generation & Create an image according to a textual prompt\\
Image editing & Edit image based on the textual prompt\\
Face detection & Detect human faces in given images and output the bounding boxes\\
Python package & Various packages such as `matplotlib' and `opencv'\\
 \hline
\end{tabular}
\end{center}
\vskip -0.2in
\end{table}





\subsection{Training}
\vskip -0.1in
Given a data point  
$\{ F_{\text{opt}}, Q, \{t_1, \cdots, t_n\}, \{c_1, \cdots, c_n\}, \{o_1, \cdots, o_n\}, A \}$, we train the VLM controller using the cross-entropy loss,
\vskip -0.15in
\begin{equation}
\begin{aligned}
\min \mathbb{E}_{(F_{\text{opt}}, Q, {\color{red}T}, C, O, A)\sim \mathbb{D} }\left[ - \sum_{i=1}^{n} P({\color{red}t_i}, c_i| F_{\text{opt}}, Q, h_i)\right],
\end{aligned}
\end{equation}
\vskip -0.1in
where $\mathbb{D}$ is the collected MM-Traj dataset and we sum the loss values of the $n$ steps in the trajectory. 
Note that, in training VLMs, we do not use the final answer $A$, as we encourage the controller to leverage tools in solving given tasks, instead of directly producing an answer based on its internal knowledge.
% which is consistent with our goal: improving the tool-usage capability of the agent instead of enriching its common knowledge.
After training, we obtain the T3-Agent.

\textbf{Model.} We use the same model architectures as MiniCPM-V-8.5B \citep{yao2024minicpm} and {\color{red}Qwen2-VL-7B}~\citep{wang2024qwen2} as our VLM controllers, including their visual encoders, resamplers, and LLMs.
We initialize the model using their released versions.

% , having 8.5B parameters. Our model uses SigLIP SoViT-400m/14\citep{zhai2023sigmoid} as the visual encoder and employs a perceiver resampler structure with one-layer cross-attention as the visual token compressor. This visual token compressor reduces the number of image tokens to 64, which allows the model to train on a long context window and multi-image settings. Our model uses Qwen-2-7B \citep{qwen2} as the language model backbone, which supports the 32k context window.

\section{Experiments}
\vskip -0.1in

\subsection{Setting}
\vskip -0.1in

To evaluate the effectiveness of the proposed multi-modal agent tuning method, we evaluate the T3-Agent on the GTA~\citep{wang2024gta} and GAIA~\citep{mialon2023gaia} benchmarks and compare it with agents that use closed-source models (GPT-4, GPT-4o, and Claude3) and open-source models (LLaMA-3-70B-instruct~\citep{dubey2024llama}, Qwen1.5-72B-chat~\citep{bai2023qwen}, {\color{red}LLaVA-NeXT-8B~\citep{liu2024llavanext}, InternVL2-8B~\citep{chen2024far}, Qwen2-VL-7B~\citep{wang2024qwen2}}, and MiniCPM-V-8.5B~\citep{yao2024minicpm}) as the controllers. 
% Concretely, we compare the T3-Agent with Trase Agent~\citep{2024trase}, Multi-Agent~\citep{wu2023autogen}, FRIDAY~\citep{wu2024copilot}, Sibyl Agent~\citep{wang2024sibyl}, and Lego Agent~\citep{AgentLego_Contributors_AgentLego_Open}.
Concretely, we compare the T3-Agent with Lego Agent~\citep{AgentLego_Contributors_AgentLego_Open}, Sibyl Agent~\citep{wang2024sibyl}, and the Warm-up Act Agent~\citep{mialon2023gaia}.
% We also report the performance of agents from the leaderboard of GAIA~\citep{mialon2023gaia}, including AgentIM, Warm-up Act, DAS Agent, and MMAC.
The huggingface agent (HF Agent)~\citep{huggingfaceagent} is the baseline agent, using the same tools as the T3-Agent.
We conduct ablation experiments to evaluate our data synthesis pipeline and visualize the task-solving process of our T3-Agent.



\textbf{Training.} To preserve the visual perception and reasoning capabilities of MiniCPM-V and Qwen2-VL, we combine the training data in MM-Traj with the data in Cauldron~\citep{lindstrom2022clevr} and open-LLaVa-NeXT~\citep{openllava1m} datasets. We train $5$ epoch over all data.
In the training process of our VLM controller, we freeze the vision encoder and visual token compressor, and fine-tune the language model using LoRA~\citep{hu2021lora}. We set the rank as 64 and apply LoRA on query, key, and value projection matrices in all self-attention layers. 
% This setting involves 7.5\% of parameters of MiniCPM-V 2.6. 
We use the AdamW optimizer with a cosine annealing scheduler. The learning rate is $1e-6$ and the batch size is 2. We set the max context window to 10240 to support the long trajectory of our agent. 

\textbf{Benchmark.} 
GTA and GAIA benchmarks are comprehensive evaluation benchmarks for multi-modal agents. 
GTA contains 229 tasks with 252 images, and the steps required to solve tasks range from 2 to 8, with most questions requiring 2 to 4 steps. It requires multi-modal agents to build powerful perception, operation, logic, and creativity abilities on visual data.
In addition to visual data, diverse files (such as PPTX, PDF, XLSX files, \emph{etc}) are also commonly encountered in practical multi-modal tasks. To evaluate agents on such files, we use the GAIA benchmark that contains 446 tasks with 109 files. The tasks in GAIA are divided into three levels, the steps of which range from 2 to arbitrarily long sequences, evaluating the capabilities of document understanding, web surfing, logic reasoning, and answer summarization. 


\textbf{Metric.} 
In the GTA benchmark, we measure three metrics for agents, including \emph{AnsAcc}, \emph{ToolAcc}, and \emph{CodeExec}.
\emph{AnsAcc} measures the correctness of predicted answers.
\emph{ToolAcc} means the accuracy of tool selection and answer summary.
\emph{CodeExec} quantifies the percentage of generated codes that could be executed without errors.
In the GAIA benchmark, we measure \emph{AnsAcc} of its three levels.
% \emph{AnsAcc} is measured using the intrinsic metric in the two benchmarks, while the latter two metrics are checked manually.


\begin{table}[t]
\caption{Results on the GTA benchmark}
\label{table:experiment_GTA}
\begin{center}
\small
\begin{tabular}{c c | c c c}
\hline
\multicolumn{1}{c}{\bf Method} & \multicolumn{1}{c|}{\bf Controller} &\multicolumn{1}{c}{\emph{AnsAcc}} &\multicolumn{1}{c}{\emph{ToolAcc}} &\multicolumn{1}{c}{\emph{CodeExec}} \\ \hline 
Lego Agent & GPT-4 & 46.59 & - & - \\
Lego Agent & GPT-4o &  41.52 & - & - \\
Lego Agent & GPT-3.5-turbo & 23.62 & - & - \\
Lego Agent & Claude3-opus & 23.44 & - & - \\
Lego Agent & Qwen1.5-72B-chat & 13.32 & - & - \\ 
Lego Agent & LLaMA3-70B-instruct & 8.32 & - & - \\
HF Agent & GPT-4o & 57.05 & 63.41 &	95.12 \\
HF Agent & GPT-4o mini & 57.69 & 56.10 & 100.00 \\
\hline
% \hline
{\color{red}HF Agent} & {\color{red}LLaVA-NeXT-8B} & {\color{red}14.10} & {\color{red}14.97} & {\color{red}25.08} \\
{\color{red}HF Agent} & {\color{red}InternVL2-8B} & {\color{red}32.05} & {\color{red}36.75} & {\color{red}52.18} \\
HF Agent & MiniCPM-V-8.5B & 33.97 & 36.59 & 56.10 \\
{\color{red}HF Agent} & {\color{red}Qwen2-VL-7B} & {\color{red}42.31} & {\color{red}44.85} & {\color{red}65.19} \\
\hline
\bf T3-Agent & Tuned MiniCPM-V-8.5B & 52.56 & 65.85	& 80.49 \\
\bf {\color{red}T3-Agent} & {\color{red}Tuned Qwen2-VL-7B} & {\color{red}53.85} & {\color{red}64.63} & {\color{red}84.32} \\
\hline
\end{tabular}
\end{center}
\vskip -0.25in
\end{table}



\subsection{GTA Results}
\vskip -0.1in
The performance of agents on the GTA benchmark is shown in~\cref{table:experiment_GTA}, where \emph{AnsAcc}, \emph{ToolAcc}, and \emph{CodeExec} are reported. 
Our agent achieves better results than the Lego agent that uses closed-source models (\emph{e.g.}, GPT-4 and GPT-4o) and HF agent using open-source models (\emph{e.g.}, InternVL2-8B), showing its effectiveness in solving complex tasks. 
The comparison of agents using the tuned and untuned VLMs shows the effectiveness of our multi-modal agent tuning method. 
For example, tuning MiniCPM-V-8.5B leads to about $18 \%$, $29 \%$, and $24 \%$ improvements on the answer accuracy, tool correctness, and code executability, respectively.
In addition, compared to the HF agent using GPT-4o and GPT-4o mini, our agent has higher \emph{ToolAcc} while lower \emph{CodeExec}, showing that our tuned VLM has more powerful reasoning capability for tool usage, while the weak programming capability results in worse \emph{AnsAcc}. This inspires us to develop VLMs for writing codes.



% \begin{table}[t]
% \caption{Results on the GTA benchmark using tools in the Lego Agent}
% \label{table:experiment_GTA}
% \begin{center}
% \begin{tabular}{c | c c c c | c c c c c}
% \multicolumn{1}{c}{\bf Method} & \multicolumn{1}{c}{\bf Inst.} & \multicolumn{1}{c}{\bf Tool.}  & \multicolumn{1}{c}{\bf Arg.}  & \multicolumn{1}{c}{\bf Summ.}  \multicolumn{1}{c}{\emph{P.}} &\multicolumn{1}{c}{\emph{O.}} &\multicolumn{1}{c}{\emph{L.}} &\multicolumn{1}{c}{\emph{C.}} & \multicolumn{1}{c}{\emph{Ans.}} 
% \\ \hline 
% GPT-4o \\
% GPT-4o-mini \\
% \hline
% MiniCPM-V \\
% \bf T3-Agent \\
% \hline
% \end{tabular}
% \end{center}
% \end{table}


\begin{table}[t]
\caption{Results on the validation set of the GAIA benchmark}
\label{table:experiment_gaia_val}
\begin{center}
\small
% \resizebox{1\columnwidth}{!}{
\begin{tabular}{c c | c c c c }
\hline
\multicolumn{1}{c}{\bf Method} & \multicolumn{1}{c|}{\bf Controller} &\multicolumn{1}{c}{\emph{AnsAcc}}  &\multicolumn{1}{c}{\emph{Level 1}} & \multicolumn{1}{c}{\emph{Level 2}} & \multicolumn{1}{c}{\emph{Level 3}} 
\\ \hline 
% Trase Agent & GPT-4o & 40.0 & 47.17  & 40.7 & 23.1   \\
% AgentIM & GPT-4-turbo & 40.0 & 50.9 & 40.7 & 15.4  \\
% Multi-Agent & GPT-4-turbo & 39.4 & 54.7 & 38.4 & 11.5  \\
% FRIDAY & GPT-4-turbo &  34.6 & 45.3 & 34.9 & 11.5   \\
Sibyl Agent & GPT-4-turbo & 29.70 & 43.40 & 27.90 & 7.70  \\
Warm-up Act & GPT-4-turbo & 17.60 &30.20 & 15.10 & 0.00 \\
% \hline
HF Agent & GPT-4o & 33.40 & 47.17 &	31.40 & 11.54  \\
HF Agent & GPT-4o mini & 26.06 & 33.96 & 27.91 & 3.84  \\
\hline
{\color{red}HF Agent} & {\color{red}LLaVA-NeXT-8B} & {\color{red}3.64} & {\color{red}9.43} & {\color{red}1.16} & {\color{red}0.00}  \\
{\color{red}HF Agent} & {\color{red}InternVL2-8B} & {\color{red}4.85} & {\color{red}7.55} & {\color{red}4.65} & {\color{red}0.00} \\
% \hline
HF Agent & MiniCPM-V-8.5B & 7.27 & 13.21 &	5.81 &	0.00 \\
{\color{red}HF Agent} & {\color{red}Qwen2-VL-7B} & {\color{red}9.70} &	{\color{red}16.98} & {\color{red}8.14} & {\color{red}0.00} \\
\hline
\bf T3-Agent & Tuned MiniCPM-V-8.5B & 15.15 & 26.42 & 11.63 & 3.84  \\
\bf {\color{red}T3-Agent} & {\color{red}Tuned Qwen2-VL-7B} & {\color{red}16.97} & {\color{red}26.42} & {\color{red}15.12} & {\color{red}3.84}\\
\hline
\end{tabular}
% }
\end{center}
\vskip -0.25in
\end{table}


\subsection{GAIA Results}
\vskip -0.1in
In~\cref{table:experiment_gaia_val}, we report the performance of T3-Agent on the validation set of GAIA.
% including the \emph{AnsACC} and accuracies on the three levels. 
T3-Agent performs better than agents driven by open-source models. For example, Qwen2-VL-7B achieves the best performance among all open-source models, while our agent is still $7\%$ higher than it.
The performance improvements across multiple VLMs validate the effectiveness of our dataset.
% In addition, T3-Agent has comparable performance with the Warm-up Act agent that uses the powerful GPT-4-turbo model. 
{\color{red}Compared with agents driven by closed-source models (\emph{e.g.}, GPT-4), our T3-Agent achieves worse performance. The reason is that closed-source models use larger model sizes and more training data. These factors may primarily contribute to the performance differences.}







% \begin{table}[t]
% \caption{Results on the test set of the GAIA benchmark}
% \label{table:experiment_gaia_eval}
% \begin{center}
% \resizebox{1\columnwidth}{!}{
% \begin{tabular}{c c | c c c c | c c c}
% \hline
% \multicolumn{1}{c}{\bf Method}  & \multicolumn{1}{c|}{\bf Controller} &\multicolumn{1}{c}{\emph{AnsAcc}}  &\multicolumn{1}{c}{\emph{Level 1}} & \multicolumn{1}{c}{\emph{Level 2}} & \multicolumn{1}{c}{\emph{Level 3}} & \multicolumn{1}{c}{\emph{ToolAcc}} &\multicolumn{1}{c}{\emph{CodeExec}} &\multicolumn{1}{c}{\emph{CodeAcc}} 
% \\ \hline 
% Trase Agent & GPT-4o & 35.6 & 50.5 & 33.3 & 14.3  & - & - & - \\
% Sibyl Agent & GPT-4o & 34.6 & 47.3 & 32.7 & 16.3 & - & - & -\\
% DAS Agent & GPT-4o & 32.3 & 47.3 & 28.3 & 16.7 & - & - & -\\
% Multi-Agent& GPT-4-turbo & 32.3 & 47.3 & 28.9 & 14.6 & - & - & -\\
% MMAC & GPT-4V & 25.9 & 45.2 & 20.8 & 6.1 & - & - & -\\
% \hline
% HF Agent &  GPT-4o \\
% HF Agent & GPT-4o mini  \\
% HF Agent & MiniCPM-V  \\
% \bf T3-Agent & Tuned MiniCPM-V \\
% \hline
% \end{tabular}
% }
% \end{center}
% \end{table}


\begin{wraptable}{r}{0.5\textwidth}
\vspace{-12mm}
% \begin{table}
\begin{center}
\caption{Average scores from humans.}
\label{table:human_verification}
\centering
% \tiny
% \resizebox{1\columnwidth}{!}{
% \setlength{\tabcolsep}{1pt}
\begin{tabular}{c c | c c }
    \bottomrule
    \multicolumn{2}{c |}{MM-Traj} & \multicolumn{2}{c}{Filtered out Data} \\
    Task & Trajectory & Task & Trajectory \\    \hline
    {\color{red}8.32} & {\color{red}8.67} & {\color{red}6.36} & {\color{red}6.38} \\
    % \hline
    \bottomrule
\end{tabular}
\end{center}
% \end{table}
\vspace{-5mm}
\end{wraptable}

\subsection{Data Quality}
\vskip -0.1in
To evaluate the data quality of generated data in MM-Traj, we conduct a user study. 
{\color{red}Concretely, we randomly sample 600 data points from the MM-Traj datasets and filtered out data. We ask 30 persons (with rich programming experience) to provide scores (1-10) for the task quality and trajectory quality, and they do not know whether the data is from MM-Traj or filtered out data.}
We ask the persons to provide scores for the tasks (the queries and files) and trajectories.
% ``Please consider the quality of the task (the query and files). The score is in the range (1-10), where 1 means its quality is bad and 10 means its quality is very good".
% Then, we ask the person ``Please consider the trajectory quality to solve the task. 
The score is in the range (1-10), where higher scores mean better quality.
% 1 means its quality is bad and means its quality is very good". 
Results are shown in~\cref{table:human_verification}. The quality of MM-Traj is higher than the filtered-out data, demonstrating the used verifiers can discard lower-quality data.




\begin{wraptable}{r}{0.47\textwidth}
\vspace{-9mm}
\caption{Ablation}
\label{table:experiment_ablation}
\begin{center}
\begin{tabular}{c c c}
\hline
\multicolumn{1}{c}{\bf Method}  &\multicolumn{1}{c}{\bf GTA} &\multicolumn{1}{c}{\bf GAIA}
\\ \hline 
w/o two verifier & 50.00 & 13.33\\
Ours (two verifiers) & 52.56 & 15.15\\
\hline
\end{tabular}
\end{center}
\vspace{-5mm}
\end{wraptable}


\begin{figure}[]
\begin{center}
    \includegraphics[width=0.9\linewidth]{figure/visualization.pdf}
    % \vskip -0.1in
    \caption{Case study of the T3-Agent in the GTA benchmark.}
    \vskip -0.2in
    \label{fig:data_visualization}
\end{center}
\end{figure}


\subsection{Ablation}
\vskip -0.1in
We conduct ablation experiments to evaluate the effectiveness of our two verifiers, as shown in~\cref{table:experiment_ablation}. We observe that on both the two benchmarks, the data using the two verifiers leads to better performance (\emph{e.g.}, $2.56 \%$ improvements on the GTA benchmark), showing the effectiveness of the two verifiers.




\subsection{Visualization}
\vskip -0.1in
In~\cref{fig:data_visualization} and~\cref{fig:data_visualization2}, we visualize cases solved by our T3-Agent in the GTA and GAIA benchmarks. We have the following conclusions. (1) Our agent could handle multiple-image reasoning tasks. By utilizing the visual information from given images, the agent could apply the correct tools and write correct arguments for given images. (2) Our agent could solve complex tasks requiring long code. (3) Our agent could revise code errors based on observations. 
(4) T3-Agent can solve tasks with multi-hop questions. For example, in the first case of~\cref{fig:data_visualization2}, our agent searches for information from the web, based on obtained information in the first step.
(5) T3-Agent could handle multi-modal files, such as audio and PDF files in~\cref{fig:data_visualization2}.






\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.9\linewidth]{figure/visualization2.pdf}
    \vskip -0.1in
    \caption{Case study of the T3-Agent in the GAIA benchmark.}
    \vskip -0.2in
    \label{fig:data_visualization2}
\end{center}
\end{figure}

\section{Conclusion}
\vskip -0.1in
In this paper, we have presented a multi-modal agent tuning method that improves the tool-usage capability of agents by generating a large number of tool-usage data and tuning a VLM using these data. 
Given proper prompts and sufficient source images, our data synthesis pipeline can produce high-quantity multi-modal tasks with trajectories. 
We collect these generated data into an MM-Traj dataset to tune a MiniCPM-V model, and the T3-Agent with the tuned model has achieved significant improvements on two multi-modal benchmarks, demonstrating the effectiveness of the data synthesis pipeline and the collected MM-Traj dataset. 

\textbf{Limitation.} 
In the current T3-Agent, we only consider the multi-modal information in queries. Practical tasks usually involve multi-modal data in trajectories of agents, such as the intermediate results in image editing tasks. We will study how to utilize multi-modal information in agent trajectories, which benefits in performing more powerful step-by-step reasoning for tool usage.
% In addition, the current data synthesis pipeline fixes the toolset for all tasks. Such an assumption is hard to satisfy. 









